SRACARE: Secure Remote Attestation with Code Authentication and Resilience Engine

Recent technological advancements have enabled proliferated use of small embedded and IoT devices for collecting, processing, and transferring the security-critical information and user data. This exponential use has acted as a catalyst in the recent growth of sophisticated attacks such as the replay, man-in-the-middle, and malicious code modification to slink, leak, tweak or exploit the security-critical information in malevolent activities. Therefore, secure communication and software state assurance (at run-time and boot-time) of the device has emerged as open security problems. Furthermore, these devices need to have an appropriate recovery mechanism to bring them back to the known-good operational state. Previous researchers have demonstrated independent methods for attack detection and safeguard. However, the majority of them lack in providing onboard system recovery and secure communication techniques. To bridge this gap, this manuscript proposes SRACARE- a framework that utilizes the custom lightweight, secure communication protocol that performs remote/local attestation, and secure boot with an onboard resilience recovery mechanism to protect the devices from the above-mentioned attacks. The prototype employs an efficient lightweight, low-power 32-bit RISC-V processor, secure communication protocol, code authentication, and resilience engine running on the Artix 7 Field Programmable Gate Array(FPGA) board. This work presents the performance evaluation and state-of-the-art comparison results, which shows promising resilience to attacks and demonstrate the novel protection mechanism with onboard recovery. The framework achieves these with only 8 % performance overhead and a very small increase in hardware-software footprint.

==> discussion.tex <==
\section{Discussion} \label{discussion}
\subsection{Limitations and Countermeasures}
A possible criticism of this work is that booting from an SD card or USB Flash provides the same level of protection. We have listed a few reasons to justify our design chosen. The first is that providing physical security for the SD card or USB flash is extremely difficult. Users can take the disks wherever they like and change content, add malicious software, get lost, or get into the hands of suspicious actors. Those actors can add or replace any hardware or software module into the system without security controls or add privilege levels to access other secure resources. The second issue could be to store the golden image on EEPROM and not on flash or other storage on board. Attacks like buffer overflow \cite{bumping}, \cite{Rootkit:2019}, \cite{buffer:2000} have showcased that attacking the same memory module is relatively easy compared to attacking different memory module located at a different location and has different read-write access control. Also, recent technological advancement had made EPROM cost significantly low (e.g., $< .50$ cents for 32KB when buying in bulk), which makes it a right candidate for proposed work. To reduce the size of data stored in EEPROM  memory, one can have only mission-critical boot flash codes like initial drivers and hardware setup for networking stack or SPI, I2C interface through which remote access can be possible to reflash the device. However, opening network access for reflashing brings a whole new area of attacks to protect against malicious actors reflashing the system.
The last possible concern is why communication is not done with an internal fast system bus and using SPI connection. SPI is relatively slow compared to the interconnect bus. However, SPI has a dedicated connection to flash and bootstrapping hosts, which reduces the attack surface from other malicious hardware-software resources. Lastly, the choice of the symmetric cryptographic core can make the key propagation hard for large embedded systems. We have used symmetric cryptography over asymmetric due to a light hardware footprint.   
\subsection{Future Research}
Future work on \emph{SRACARE} focuses on having a hardware compression unit to compress the flash data, explore the possibility of storing data into protected flash or on a one-time programmable memory region. We also plan to explore the onboard attestation trigger and mitigation mechanism to avoid the need of RA to verify the integrity and authenticity of the device. The secure SoC presented in this work can be placed as a separate boot processor (or co-processor like TPM) on any platform, including large computer systems, servers, or devices. The secure boot with resilience design on a dedicated boot processor gives the added advantage of the separating attack surface and increase security.


==> performance.tex <==
\section{System Performance Analysis}
\subsection{Chain of Trust}
 First secure bootstrap with integrity assurance was proposed in "AEGIS" \cite{Arbaugh:1997}. The integrity of a layer during the boot process can only be guaranteed if and only if two rules are followed. (1) The integrity of the lower layers is checked. (2) Transitions to higher layers occur only after integrity checks on lower layers are complete.\\ 
Convensional secure boot measures the boot integrity of each stage of boot code at file level. This implementation uses the same concept but in different data context. This work takes 1 KB chunks of flash code for integrity measurement. The chain of trust is represented the following way, 
\[ 
I_0{} = True 
\]
\begin{equation}
I\textsubscript{i+1} = I_i{}\;\;\;\; \& \;\;\;\; V_i{}(L\textsubscript{i+1} )
\end{equation}
$I_i{}$ is a boolean value representing the integrity of level i, and \& is the boolean AND operation. $V_i{}$ is the verification function associated with the $i^{th}{}$ layer. $V_i{}$ takes as its only argument the level to verify, and it returns a boolean value as a result. The verification function performs a cryptographic hash of the frame and compares the result to stored digest value. As explained earlier, this work has divided boot flash data into 1 KB frame chunks and hash is computed on each frame for verification. Therefore, we represent the recurrence to:
\[ 
I_0{} = True 
\]
\begin{equation}
   I\textsubscript{i+1} =\left\{
                \begin{array}{ll}
                  I_i{}  \;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\; for \;\; i = 0\\
                  I_i{} \;\; \& \;\; V_i{}  (L\textsubscript{i+1} ) \;\;\;\;\;\;\;\;\;\;\;\;\;    for \;\; i = 1\\
                  I_i{} \;\; \& \;\; \sum_{i=2}^{n} V_i{} (L\textsubscript{i+1}) \;\;\;for \;\; i = 2,3 ...n\\
                  
                \end{array}
              \right.
 \end{equation}
Here, $I_0{}$ is boot ROM code assumed to be trusted. $I_1{}$ is the first frame which will be handled differently as explained in subsection 4.2. n represents the number of frames of flash image. 
\subsection{Performance Analysis}
Using the recurrance relation shown in equation 2, one can compute the estimated increase in boot time (T\textsubscript{$\Delta$}) with secure boot without integrity failures.  
\begin{equation}
T\textsubscript{$\Delta$} = t\textsubscript{fm}(V_0{}(L_1{}))\;\; + t\textsubscript{fm}(\sum_{i=1}^{n}V_i{}(L_{i+1}{}))
\end{equation}
Where t\textsubscript{fm} is execution time for each frame. The verification time includes time required to compute SHA256 message digest and time required to compare it against pre-computed hash. As explained in frame structure, this work first matches the frame number for first frame and clears the flash region to reflash it with trusted code. Therefore, the time required for the first frame processing is different than remaining frames. 

\subsubsection{Performance analysis of HW v/s SW HMAC-SHA256}
\par The performance analysis of hardware and software implementation of the main module HMAC-SHA256 is performed in two steps. At first, the resource utilization in terms of speed, throughput, energy consumption, and energy efficiency are calculated from static and dynamic power analysis from the hardware and software implementation running on FPGA. The comparison is depicted in Table.1. This implementation uses a block size of 256-bit for the HMAC-SHA256 calculation.
\begin{table}[h]\caption{Hardware software performance analysis of HMAC-SHA256 on FPGA.}
	\scalebox{1.3}[1.3]{
	\begin{tabular}{@{}lcc@{}}
	\toprule
	\multicolumn{3}{c}{Performance Analysis of HMAC-SHA256 on FPGA}  \\ \midrule
	\multicolumn{1}{l|}{Parameters}              & \multicolumn{1}{c|}{Software} & Hardware \\ \midrule
	\multicolumn{1}{l|}{Cycles (c)}         & \multicolumn{1}{c|}{47033}   &  2926   \\
	\multicolumn{1}{l|}{Frequency (f)(MHz}            & \multicolumn{1}{c|}{100}   & 100    \\
	\multicolumn{1}{l|}{Block (b)} & \multicolumn{1}{c|}{256}      & 256    \\
	\multicolumn{1}{l|}{Throughtput T(Mbps)}     & \multicolumn{1}{c|}{.54}    & 8.74   \\
	\multicolumn{1}{l|}{Time(usec)}           & \multicolumn{1}{c|}{470.33}       & 29.26    \\
	\multicolumn{1}{l|}{Energy Consumption E }                & \multicolumn{1}{c|}{197.06}       & 12.25    \\
	\multicolumn{1}{l|}{Energy Efficiency}      & \multicolumn{1}{c|}{92.68}    & 0.358    \\ \bottomrule
	\end{tabular}
	}\label{tab:hwswperf}
	\vspace{-3mm}
\end{table}   
\subsubsection{Timing analysis of bootstrapping}
\par The results indicates that performance is increased by 16x and 92${\%}$ less power is utilized on hardware HMAC-SHA256. Therefore, the hardware HMAC-SHA256 module is selected for secure SoC design.    
\subsubsection{Timing analysis of bootstrapping}
\par Table.1 depicts performance analysis of hardware v/s software based HMAC-SHA256 module for only one block of data of size 256 bytes. The boot flash size is 5.6 KB for current application which is devided into six 1 KB chunks and the timing analysis is presented in Table.2. 
\par Using the equation 3 the total time T\textsubscript{$\Delta$} is calculated for with and without secure boot with resilence. As explained earlier first frame requires extra time as it clears the entire flash region and reflashes the frame region. results shows that first frame requires more cycles  and the rest of the frames requires equal number of cycles. The time presented in Table.2 is the total time T\textsubscript{$\Delta$}.
\begin{table}[H]
	\caption{Timing analysis for Bootstrap.}
	\scalebox{1.2}[1.2]{
	\begin{tabular}{@{}lcc@{}}
	\toprule
	\multicolumn{3}{c}{Timing Analysis of HMAC-SHA256 bootstrap on FPGA}  \\ \midrule
	\multicolumn{1}{l|}{Parameters}              & \multicolumn{1}{c|}{without} & With \\ \midrule
	\multicolumn{1}{l|}{Cycles req. for first frame (c)}         & \multicolumn{1}{c|}{553611}   &  576083   \\
	\multicolumn{1}{l|}{Cycles (rest of frames)(c)}       & \multicolumn{1}{c|}{103330}   & 133790    \\
	\multicolumn{1}{l|}{Total Cycles}            & \multicolumn{1}{c|}{656941 }   & 709873   \\
	\multicolumn{1}{l|}{Frequency (f)(MHz)}            & \multicolumn{1}{c|}{100}   & 100    \\
	\multicolumn{1}{l|}{Time (T)(msec)}           & \multicolumn{1}{c|}{.656}       & .709    \\ \midrule
	Time difference D\textsubscript{$\Delta$} = 52.9 msec\\ \bottomrule
	\end{tabular}
	}
	\label{tab:timeanalysis}
	\vspace{-2mm}
\end{table} 
\par From Table.2 the time difference D\textsubscript{$\Delta$} = 52.9 (msec) is calculated. which indicates that with secure boot resilence bootstrapping is taking 52.9msec extra, which is insignificant compared to the level of security and resilience it provides.  
\subsection{FPGA resource utilization}
\par Table-3 depicts FPGA resource analysis of HMAC, IBEX core, and complete SoC Chip. Fourth column shows percentage utilization of available hardware resource on Nexys Video FPGA board. 
\begin{table}[h]
	\caption{Quantitative hardware resource utilization.}
	\scalebox{1.1}[1.1]{
	\begin{tabular}{@{}lcccc@{}}
	\toprule
	\multicolumn{5}{c}{FPGA Hardware Resource Utilization Report}  \\ \midrule
	\multicolumn{1}{l|}{Parameters}              & \multicolumn{1}{c|}{Proposed Chip} & \multicolumn{1}{c|}{HMAC} & \multicolumn{1}{c|}{IBEX} & {${\%Util.}$} \\ \midrule
	\multicolumn{1}{l|}{Slice LUTs}         & \multicolumn{1}{c|}{24249}  & \multicolumn{1}{c|}{2807} & \multicolumn{1}{c|}{3581} &  18   \\
	\multicolumn{1}{l|}{LUT as logic}         & \multicolumn{1}{c|}{24081}  & \multicolumn{1}{c|}{2807} & \multicolumn{1}{c|}{3581} &  18   \\
	\multicolumn{1}{l|}{LUT as DRAM}         & \multicolumn{1}{c|}{168}  & \multicolumn{1}{c|}{0} & \multicolumn{1}{c|}{8} &  1   \\
	\multicolumn{1}{l|}{Slice Registers}         & \multicolumn{1}{c|}{19586}  & \multicolumn{1}{c|}{2312} & \multicolumn{1}{c|}{2559} &  7   \\
	\multicolumn{1}{l|}{Register as FF}         & \multicolumn{1}{c|}{19581}  & \multicolumn{1}{c|}{2312} & \multicolumn{1}{c|}{2559} &  7   \\
	\multicolumn{1}{l|}{Register as Latch}         & \multicolumn{1}{c|}{5}  & \multicolumn{1}{c|}{0} & \multicolumn{1}{c|}{0} &  $<$1   \\
	\multicolumn{1}{l|}{F7 Muxes}         & \multicolumn{1}{c|}{1407}  & \multicolumn{1}{c|}{71} & \multicolumn{1}{c|}{265} &  2   \\
	\multicolumn{1}{l|}{F8 Muxes}         & \multicolumn{1}{c|}{196}  & \multicolumn{1}{c|}{29} & \multicolumn{1}{c|}{0} &  1   \\ \bottomrule
	\end{tabular}
	}\label{tab:quanthw} 
		\vspace{-2mm}
\end{table} 
\par The FPGA implementation of HMAC-SHA256 for CARE uses 3x less area and operates at 2x faster speed when compared to other implementation from \cite{Juliato2011FPGAIO} work. The work in \cite{Haj:2019} requires 27170 Slice LUTs for only  one module (ECDSA) implementation which is 14x larger than the proposed solution. Also \cite{Haj:2019} design requires two 64 bit RISC-V cores for TEE implementation along with additional hardware of SHA3 and CoLPUF. This design choieses makes it resource heavy solution and not suitable for a small embedded or IoT devices. 

==> relatedwork.tex <==
\section{Related work} \label{Relatedwork}
\par This section gives an overview of the most common techniques for remote attestation and secure-boot. Remote attestation is a process of remotely verifying the state of the software running on the untrusted device.  RA measures the cryptographic digest of the software running on the untrusted device. We have classified previously implemented RA's into three categories: Hardware based, Software based, and Hybrid.
{\bf{Hardware Based RA}:} One of the most popular methods of RA, uses a discrete co-processor called Trusted Platform Module (TPM) \cite{Tpm:2010} recommended by Trusted Computing Group (TCG). TPM has some "special purpose registers" called Platform Configuration Registers (PCRs), which cannot be overwritten but can only be extended by hashing of software measurements together with previous PCR values. The TPM can sign the PCRs with a private attestation key to generate attestation evidence. The TPM provides hardware root-of-trust. However, due to space, size, and cost constraints, it is not suitable for small embedded or IoT devices.
\par Some researchers have used Trusted Execution Environment (TEE) \cite{Sabt:2015} or proprietary implementation of Arm TrustZone \cite{Jiang:2017}. TrustZone uses hardware-based isolation and access control between the secure world and the non-secure world. Microsoft's fTPM \cite{mcs:2015} provides a use case of TrustZone for secure boot and attestation. Intel's SGX \cite{sgx:2013} provides instruction and memory access features to instantiate protected containers referred to as enclaves by using special instructions and processor extensions. TrustZone and TEE increase design complexity and cost due to exclusive licensing. Some secure boot architectures use Unified Extensible Firmware Interface (UEFI) \cite{NSA}, which is involved in the design and not suitable for small embedded and IoT devices.\\
{\bf{Software Based RA}:} Other researchers have used simulated or software TPM implementations like simTPM \cite{Chakraborty:2019} or IBM's software TPM \cite{Goldman}. Sanctum \cite{Sanctum:2018} and \cite{ndss:2018} uses a software-based crypto engine for remote attestation. \\
{\bf{Hybrid RA}:} SMART \cite{Wong:2018} is a dynamic root-of-trust architecture for low-end devices at runtime. SPM/Sancus: SPM \cite{Stra:2010} and Sancus \cite{sancus:2013} present a security architecture which provides isolation of software modules using additional CPU instructions. TrustLite/TyTAN: TrustLite \cite{TrustLite:2014} and its successor TyTAN \cite{TyTan:2015} provide flexible, hardware-enforced isolation of software modules using Execution-Aware Memory Protection Unit (EA-MPU) in hardware.
\par Some other \mbox{RISC-V} based remote attestation and secure-boot architectures like Shakti-T \cite {Shakti:2017} uses base and bounds concept to secure pointer's access to valid memory regions. Keystone \cite{keystone} showcases a trusted execution environment (TEE) with enclaves. Lightweight, secure boot work proposed in \cite{Haj:2019} represents hardware-based secure boot. A recent opensource root-of-trust project from Google called Opentitan \cite{Ope:2019} provides a sample implementation of secure boot. However, none of the available solutions has a secure recovery mechanism. Healed \cite{Healed:2019} has demonstrated the first recovery mechanism using Merkle Hash Tree (MHT), which assumes at least one node in the network is untempered, and firmware of it can be used to reflash corrupted nodes. Another implementation \cite{Secerase:2010} has shown a method of putting software receiver-transmitter code into trusted ROM for connecting to a recovery server, which also requires additional ROM storage. The proposed method uses a different approach of storing recovery data in the backup, secure ROM for small embedded IoT applications. To the best of our knowledge, proposed work is the first implementation of a \emph{hybrid lightweight secure RA architecture with secure boot and onboard resilience engine} for RISC-V based resource-constrained embedded and IoT systems. 




